Boosting Adversarial Transferability through Enhanced Momentum

Deep learning models are known to be vulnerable to adversarial examples crafted by adding human-imperceptible perturbations on benign images. Many existing adversarial attack methods have achieved great white-box attack performance, but exhibit low transferability when attacking other models. Various momentum iterative gradient-based methods are shown to be effective to improve the adversarial transferability. In what follows, we propose an enhanced momentum iterative gradient-based method to further enhance the adversarial transferability. Specifically, instead of only accumulating the gradient during the iterative process, we additionally accumulate the average gradient of the data points sampled in the gradient direction of the previous iteration so as to stabilize the update direction and escape from poor local maxima. Extensive experiments on the standard ImageNet dataset demonstrate that our method could improve the adversarial transferability of momentum-based methods by a large margin of 11.1% on average. Moreover, by incorporating with various input transformation methods, the adversarial transferability could be further improved significantly. We also attack several extra advanced defense models under the ensemble-model setting, and the enhancements are remarkable with at least 7.8% on average.

==> method_backup.tex <==
\subsection{Motivation}
\label{sec:motivation}
As shown in Figure~\ref{fig:gradient_update}~(a), MI-FGSM \cite{dong2018boosting} accumulates the gradient of each iteration to stabilize the update direction and escape from poor local maxima, which achieves higher transferability than I-FGSM~\cite{kurakin2017IFGSM}. As depicted in Figure~\ref{fig:gradient_update} (b), NI-FGSM \textit{looks ahead} by accumulating the gradient after adding momentum to the current data point so as to converge faster and achieve higher transferability \cite{lin2020nesterov}. 

Different from typical optimization process, however, the optimization for the adversary generation has restricted the optima in the neighborhood of the original input. 
%In our opinion, it raises a new concern 
It raises us a new concern: \textit{With the accumulated momentum of NAG, the evaluated data point might exceed the neighborhood of the original input and provide imprecise gradient information, which may harm the transferability of the adversaries.} 
To address this concern, we propose a Pre-gradient guided momentum Iterative FGSM (PI-FGSM), depicted in Sec.~\ref{sec:PI-FGSM}.

% To support our hypothesis, we adopt the gradient of the previous iteration to replace the ``look ahead'' portion for NAG, denoted as Pre-gradient Iterative FGSM (PI-FGSM)
% %(see details in Appendix)
% , to craft the adversaries, which achieves higher transferability than NI-FGSM, as shown in Table~\ref{tab:comparison_inc_v3}. 

% On the other hand, the accumulated gradient of previous iterations by MI-FGSM helps achieve higher transferability, which %also raises an intriguing question:
On the other hand, though MI-FGSM and NI-FGSM accumulates the gradient of various data points in the previous iterations, they both achieve higher transferability. This
 inspires us another question: %concern: 
\textit{At each iteration, could we further improve the attack transferability by accumulating the gradients of multiple data points around the current data point for the iterative gradient-based attacks?}
To address this question, we %extend MI-FGSM to 
further add sampled data points in the direction of the gradient at the previous iteration and get
the Enhanced MI-FGSM (EMI-FGSM), as depicted in Sec.~\ref{sec:EMI-FGSM}.
% We tried RI, then tried MRI
% PMI: Pre-gradient Momentum Iterative FGSM
% RMI: Random Momentum Iterative FGSM
% ERMI: Enhanced Random Momentum Iterative FGSM
% EPMI: Enhanced Pre-gradient Momentum Iterative FGSM

% To address this question, we propose a variation of MI-FGSM called Random Momentum Iterative FGSM (RMI-FGSM), which accumulates the gradients of the examples randomly sampled from the neighborhood at each iteration rather than just use the gradient of the current data point as in MI-FGSM. As shown in Table~\ref{tab:comparison_inc_v3}, though its white-box attack success rates 
% %has a little decrease
% slightly decay, the transferability of RMI-FGSM is even better than PI-FGSM, especially on the adversarially trained models. The details of PI-FGSM and MRI-FGSM are provided in Appendix~\ref{sec:variation}.

% The above analysis and the performance gain of the two methods inspire us to combine the advantages of PI-FGSM and RMI-FGSM for the sake of enhancing the transferability of the generated adversarial examples. We provide details of the enhanced momentum iterative methods (EMI-FGSM) in Sec. \ref{sec:EMI-FGSM}.
% Based on the above analysis, we propose Enhanced Momentum Iterative Methods by combining the PI-FGSM and RMI-FGSM to boost the adversarial attacks. We provide the details of Enhanced Momentum Iterative Fast Gradient Sign Method (EMI-FGSM) as in Sec.\ref{sec:EMI-FGSM}. It is notable that our methods is generally applicable to any iterative gradient-based attacks.

\subsection{Pre-gradient guided Momentum based Attack}
\label{sec:PI-FGSM}
As discussed in Sec.~\ref{sec:motivation}, the accumulated momentum of NAG might adopt the gradient of data point that violates the restriction for adversarial examples, leading to comparatively low transferability. 
%To address this issue, 
To this end, we propose Pre-gradient guided momentum Iterative FGSM (PI-FGSM), which \textit{looks ahead} by the gradient of the previous iteration. Specifically, as shown in Figure \ref{fig:gradient_update} (c), PI-FGSM accumulates the gradient of data point obtained by adding the previous gradient to the current data point at each iteration.
% adopts the gradient of the previous iteration to replace the ``look ahead'' portion that use the accumulated momentum for NAG as in Eq. \ref{eq:NAG}. 
The update procedure can be summarized as:
\begin{gather}
    \tilde{x}_t^{adv} = x_t^{adv} + \alpha \cdot \tilde{g}_{t-1},\quad
    \tilde{g}_{t}=\nabla_{\tilde{x}_t^{adv}} J_f(\tilde{x}_t^{adv}, y), \nonumber \\
    g_{t} = \mu \cdot g_{t-1} + \frac{\tilde{g}_{t}}{\|\tilde{g}_{t}\|_1},\quad
    x_{t+1}^{adv} = x_t^{adv} + \alpha \cdot \text{sign}(g_{t}), \nonumber
\end{gather}
where $\tilde{g}_{t-1}$ denotes the gradient of previous iteration.

\subsection{Enhanced Momentum based Attack}
\label{sec:EMI-FGSM}
To address the second question in Sec.~\ref{sec:motivation}, we enhance the momentum by not only memorizing all the past gradients during the iterative process, but also accumulating the gradients of the sampled examples. Inspired by PI-FGSM, to help sample more helpful data points for the gradient calculation, we sample data points in the gradient direction of the previous iteration. Specifically, as shown in Figure~\ref{fig:gradient_update} (d), we calculate the gradient of the $t$-th iteration as follows:
%  instead of randomly sampling examples in the neighborhood of the input as in RMI-FGSM,
\begin{gather}
    \bar{x}_t^{adv}[i] = x_t^{adv} + c_i \cdot \bar{g}_{t-1} \label{eq:sample_data} \\
    \bar{g}_{t} = \frac{1}{N}\sum_{i=1}^N \nabla_{\bar{x}_t^{adv}[i]} J_f(\bar{x}_t^{adv}[i], y),
    \label{eq:gradient}
\end{gather}
% \begin{equation}
%     \bar{g}_{t+1} = \frac{1}{N}\sum_{i=1}^N \nabla_{(x_t^{adv}+c_i \cdot \bar{g}_t)} J_f(x_t^{adv}+c_i \cdot \bar{g}_t, y),
%     \label{eq:gradient}
% \end{equation}
where $N$ is the sampling number, $\bar{g}_{t-1}$ is the gradient calculated by the previous iteration and $c_i$ is the $i$-th coefficient sampled in interval $[-\eta, \eta]$. We denote such accumulated gradient as the enhanced momentum.

Note that enhanced momentum is generally applicable to any iterative gradient-based attacks, such as I-FGSM \cite{kurakin2017IFGSM}, PGD \cite{madry2018pgd}, and the ensemble-model attack~\cite{liu2017delving}. Here we %integrate 
incorporate the enhanced momentum into I-FGSM, denoted as Enhanced Momentum I-FGSM (EMI-FGSM), to craft highly transferable adversarial examples. The update procedure can be summarized as:
\begin{gather}
    g_{t} = \mu \cdot g_{t-1} + \frac{\bar{g}_{t}}{\|\bar{g}_{t}\|_1}, \label{eq:momentum_update} \\
    x_{t+1}^{adv} = x_t^{adv} + \alpha \cdot \text{sign}(g_{t}), \label{eq:adv_update}
\end{gather}
where $\bar{g}_{t}$ is the gradient calculated by Eq.~\eqref{eq:gradient}. The algorithm of EMI-FGSM is summarized in Algorithm~\ref{alg:EMI-FGSM}.


==> tables/transformation_single_model.tex <==
\begin{table*}[tb]
\begin{center}
\resizebox{\textwidth}{!}{
 \scalebox{0.9}{
\begin{tabular}{l|l|ccccccc}
\hline
Model & Attack & Inc-v3 & Inc-v4 & IncRes-v2 & Res-101 & Inc-v3$_{ens3}$ & Inc-v3$_{ens4}$ & IncRes-v2$_{ens}$\\
\hline\hline
\multirow{8}{*}{Inc-v3} & DIM & ~~99.0* & 64.6 & 60.9 & 52.1 & 18.3 & 17.7 & ~~9.5 \\
 & EMI-DIM (\textbf{Ours}) & \textbf{~~99.1*} & \textbf{83.5} & \textbf{78.0} & \textbf{70.6} & \textbf{27.8} & \textbf{26.0} & \textbf{13.4} \\
\cline{2-9}
 & TIM & \textbf{100.0*} & 47.0 & 44.5 & 40.5 & 24.3 & 22.0 & 13.2 \\
 & EMI-TIM (\textbf{Ours}) & \textbf{100.0*} & \textbf{79.4} & \textbf{76.3} & \textbf{67.2} & \textbf{44.3} & \textbf{40.8} & \textbf{26.2} \\
\cline{2-9}
 & SIM & \textbf{100.0*} & 70.3 & 68.0 & 62.4 & 32.4 & 30.8 & 17.2 \\
 & EMI-SIM (\textbf{Ours}) & \textbf{100.0*} & \textbf{91.9} & \textbf{90.0} & \textbf{85.4} & \textbf{45.2} & \textbf{41.8} & \textbf{23.8} \\
 \cline{2-9}
 & DTS & ~~98.9* & 83.1 & 80.7 & 75.8 & 65.2 & 62.7 & 46.0 \\
 & EMI-DTS (\textbf{Ours}) & \textbf{~~99.6*} & \textbf{94.1} & \textbf{92.6} & \textbf{89.4} & \textbf{78.9} & \textbf{75.3} & \textbf{60.4} \\
\hline\hline
\multirow{8}{*}{Inc-v4} & DIM & 74.1 & ~~98.5* & 66.3 & 58.0 & 22.3 & 21.0 & 11.6 \\
 & EMI-DIM (\textbf{Ours}) & \textbf{89.4} & \textbf{~~99.1*} & \textbf{83.6} & \textbf{75.2} & \textbf{33.5} & \textbf{30.9} & \textbf{16.7} \\
\cline{2-9}
 & TIM & 58.0 & ~~99.5* & 47.2 & 42.8 & 25.9 & 24.0 & 16.9 \\
 & EMI-TIM (\textbf{Ours}) & \textbf{89.0} & \textbf{~~99.8*} & \textbf{81.2} & \textbf{72.3} & \textbf{52.1} & \textbf{48.3} & \textbf{35.2} \\
\cline{2-9}
 & SIM & 80.6 & ~~99.5* & 73.6 & 68.8 & 47.9 & 44.9 & 29.2 \\
 & EMI-SIM (\textbf{Ours}) & \textbf{96.4} & \textbf{~~99.9*} & \textbf{93.7} & \textbf{89.0} & \textbf{59.7} & \textbf{56.1} & \textbf{36.9} \\
  \cline{2-9}
 & DTS & 84.7 & ~~98.0* & 80.5 & 76.3 & 67.9 & 66.9 & 54.3 \\
 & EMI-DTS (\textbf{Ours}) & \textbf{95.7} & \textbf{~~99.4*} & \textbf{94.5} & \textbf{90.7} & \textbf{81.4} & \textbf{77.5} & \textbf{68.8} \\
\hline\hline
\multirow{8}{*}{IncRes-v2} & DIM & 68.1 & 65.1 & ~~93.7* & 58.3 & 30.2 & 23.4 & 17.3 \\
 & EMI-DIM (\textbf{Ours}) & \textbf{88.8} & \textbf{85.1} & \textbf{~~98.5*} & \textbf{78.3} & \textbf{42.4} & \textbf{35.5} & \textbf{26.4} \\
\cline{2-9}
 & TIM & 62.1 & 55.8 & ~~97.2* & 49.9 & 31.0 & 28.3 & 21.5 \\
 & EMI-TIM (\textbf{Ours}) & \textbf{90.6} & \textbf{85.0} & \textbf{~~99.4*} & \textbf{80.1} & \textbf{61.5} & \textbf{52.2} & \textbf{48.2} \\
\cline{2-9}
 & SIM & 84.6 & 79.5 & ~~98.9* & 76.1 & 55.9 & 49.0 & 41.7 \\
 & EMI-SIM (\textbf{Ours}) & \textbf{97.5} & \textbf{95.1} & \textbf{~~99.9*} & \textbf{90.9} & \textbf{69.0} & \textbf{60.1} & \textbf{51.6} \\
  \cline{2-9}
 & DTS & 87.1 & 84.3 & ~~96.6* & 81.4 & 76.4 & 73.3 & 69.4 \\
 & EMI-DTS (\textbf{Ours}) & \textbf{97.8} & \textbf{95.4} & \textbf{~~99.9*} & \textbf{93.6} & \textbf{88.2} & \textbf{83.5} & \textbf{81.9} \\
\hline\hline
\multirow{8}{*}{Res-101} & DIM & 73.6 & 68.5 & 69.5 & ~~97.6* & 36.2 & 31.9 & 20.6 \\
 & EMI-DIM (\textbf{Ours}) & \textbf{88.7} & \textbf{84.3} & \textbf{84.1} & \textbf{~~99.7*} & \textbf{46.4} & \textbf{40.7} & \textbf{26.3} \\
\cline{2-9}
 & TIM & 59.4 & 54.0 & 52.3 & ~~99.2* & 35.6 & 31.8 & 22.8 \\
 & EMI-TIM (\textbf{Ours}) & \textbf{86.0} & \textbf{79.1} & \textbf{79.8} & \textbf{100.0*} & \textbf{56.4} & \textbf{50.3} & \textbf{41.7} \\
\cline{2-9}
 & SIM & 74.4 & 69.8 & 68.3 & ~~99.7* & 43.1 & 39.4 & 26.0 \\
 & EMI-SIM (\textbf{Ours}) & \textbf{92.0} & \textbf{88.7} & \textbf{88.4} & \textbf{100.0*} & \textbf{57.6} & \textbf{50.4} & \textbf{35.7} \\
  \cline{2-9}
 & DTS & 84.0 & 80.0 & 81.9 & ~~98.9* & 73.3 & 70.9 & 59.3 \\
 & EMI-DTS (\textbf{Ours}) & \textbf{93.7} & \textbf{90.9} & \textbf{92.3} & \textbf{~~99.6*} & \textbf{83.9} & \textbf{80.9} & \textbf{71.7} \\
\hline
\end{tabular}}}
\caption{\textbf{Attack success rates (\%) of adversarial attacks against the seven baseline models under single-model setting.} The adversarial examples are crafted on Inc-v3, Inc-v4, IncRes-v2 and Res-101, respectively.}
\label{tab:singleModel}
\end{center}
\vspace{-1.3em}
\end{table*}
